Direct sampling of short paths for contiguous partitioning

In this paper, we provide a family of dynamic programming based algorithms to sample nearly-shortest self avoiding walks between two points of the integer lattice $\mathbb{Z}^2$. We show that if the shortest path of between two points has length $n$, then we can sample paths (self-avoiding-walks) of length $n+O(n^{1-\delta})$ in polynomial time. As an example of an application, we will show that the Glauber dynamics Markov chain for partitions of the Aztec Diamonds in $\mathbb{Z}^2$ into two contiguous regions with nearly tight perimeter constraints has exponential mixing time, while the algorithm provided in this paper can be used be used to uniformly (and exactly) sample such partitions efficiently.

==> notes/analysis_for_backtracks.tex <==
% !TEX root = ../main.tex
\section{Avoiding Backtracks}
\label{s:avoiding_backtracks}
Now, we get a handle of number of walks of length $n + 2k$ from $O$ to $P = (n_1, n_2)$ without a cycle of length $2$. We will alternately refer to a cycle of length $2$ as a \emph{backtrack}, since they correspond to immediately backtracking the last step taken in the path. Note that these walks can have cycles of length $4$ or more.

We will define $W^2_k$ to be number of walks of length $n + 2k$ without any cycles of length $\le 2$, that is, without any backtracks. Let $B^2_{k,i}$ denote the number of walks of length $n + 2k$ such that deleting exactly $i$ backtracks (iteratively) gives us a walk of length $n + 2k - 2i$ without any backtracks. It is easy to see that
\begin{equation}
	\label{eq:2_good_walks_rec}
	W^2_k = W_k - \sum_{i=1}^k B^2_{k,i}
\end{equation}

Now we get a bound on $B^2_{k,i}$.
\begin{lemma}
	\label{l:2_bad_walks}
	For $k = o(\sqrt{n})$, we have the recurrence
	\begin{equation}
		\label{eq:2_bad_walks_rec}
		B^2_{k,i} = (1 + o(1)) \binom{n + 2k - i}{i} 3^i W^2_{k-i}
	\end{equation}
	as $n \to \infty$.
\end{lemma}
\begin{proof}
	By definition, given a walk of length $k$ such that deleting $i$ backtracks we can get a path of length $n + 2k - 2i$ that do not have a backtrack (but may have cycles of length $4$ or more). We now reverse this process: we start with a walk of length $n + 2k - 2i$ and add $i$ backtracks, iteratively. This process can be done as following: for each place where we can insert a backtrack (there are $n+2k-2i$ many of them), we choose the number of backtracks to add. Say we want to add $j$ backtracks at one place. Since these backtracks are nested we can denote this structure by a valid sequence of brackets. The number of those can be given by $\textsc{Cat}(j)$ where $\textsc{Cat}(j)$ denotes the $j^{\text{th}}$ catalan number. Once this configuration is fixed, we can choose the direction of each backtrack. 

	Let the choice of bracketing sequences and places to insert them be denoted by \emph{backtrack insertion scheme}. Further, each outermost bracket will be denoted as a \emph{block}. Then, the set of directions of the backtrack will be referred to as \emph{direction sequence}. We will ensure that direction sequence satisfies certain set of rules described below.

	On the other hand, if a backtrack is nested (that is, if its inside another backtrack), then its starting direction cannot be the one opposing to backtrack that contains it. For example, consider the bracketing $(())$. We can't have outer backtrack to be $UD$ and the inner one to be $DU$, since that leads to $UDUD$, which also corresponds to the bracketing $()()$.

	%TODO: can this be formalized better?

	To avoid this kind of double counting, we can allow only $3$ possibilities to any inserted backtrack. 
	\begin{enumerate}[nosep]
		\item For a outermost backtrack in a block, its direction cannot be the one opposite to the backtrack or walk direction inserted before it. 
		\item For a nested backtrack, its direction cannot be the one opposite to the backtrack that contains it, since if it is, it closes the bracket in the bracketing sequence early.
	\end{enumerate}
	These rules for the insertion imply that all but the first backtrack inserted at the very start of the walk has $3$ direction choices in the direction sequence. 

	Now, we bound the number of backtrack insertion schemes. Consider a scheme with exactly $j$ blocks. First, we insert the positions of the $j$ blocks into walk of length $n + 2k - 2i$. This can be done in $\binom{n + 2k - 2i + j}{j}$ many ways. Now, we are left with $i - j$ brackets which must be inserted inside the blocks to get a valid backtrack insertion scheme.
	The generating function for number of bracketing is given by $f_{\textsc{cat}}^j$, and we are looking for the coefficient of $x^{i-j}$. The coefficients of $f_{\textsc{cat}}^j$ are bounded by the generating function $\brac{\frac{1}{1 - 4x}}^j$, and hence we get an upper bound of 
	\begin{equation}
		\label{eq:bracket_ub}
		(-4x)^{i-j} \binom{-j}{i-j} = \binom{i}{j} 4^{i-j}
	\end{equation}
	Summing everything up, we get 
	\begin{align*}
		B^2_{k,i}
		& \le \sum_{j=1}^i \binom{n+2k-2i+j}{j} \binom{i}{j} 4^{i-j} 3^i W^2_{k-i} \\
		& \le \sum_{j=1}^i \binom{n+2k-i}{i} \frac{i^{2(i-j)}}{n^{i-j}} 4^{i-j} 3^i W^2_{k-i} \\
		& \le \binom{n+2k-i}{i} 3^i W^2_{k-i} \sum_{j=1}^i \brac{\frac{4i^2}{n}}^{i-j} \\
		& \le \binom{n+2k-i}{i} 3^i W^2_{k-i} \brac{\frac{n}{n-4i^2}} \\
		& \le (1 + o(1)) \binom{n+2k-i}{i} 3^i W^2_{k-i} 
	\end{align*}
	where the last part follows using $i \le k = o(\sqrt{n})$, giving us the result that we want.
	On the other hand, the lower bound follows from the fact that $f^j_{\textsc{cat}} \ge \brac{\frac{1}{1-x}}^j$, and a similar computation gives the lower bound
	\begin{align*}
		B^2_{k,i}
		& \ge \sum_{j=1}^i \binom{n+2k-2i+j}{j} \binom{i}{j} 3^i W^2_{k-i} \\
		& \ge \sum_{j=1}^i \binom{n+2k-i}{i} \frac{i^{2(i-j)}}{n^{i-j}} 3^i W^2_{k-i} \\
		& \ge \binom{n+2k-i}{i} 3^i W^2_{k-i} \brac{\frac{n}{n-i^2}} \\
		& \ge (1 + o(1)) \binom{n+2k-i}{i} 3^i W^2_{k-i} 
	\end{align*}
	Combining both the sides, we get the result.

	% TODO: Potential improvements in eq:bracket_ub and last computation
\end{proof}

\begin{lemma}
	\label{l:2_good_walks_bound}

\end{lemma}
\begin{proof}
	We plug in \cref{eq:2_bad_walks_rec} into \cref{eq:2_good_walks_rec} to get
	\begin{align*}
		W^2_k
		& = W_k - \sum_{i=1}^k B^2_{k,i} \\
		& = W_k - \sum_{i=1}^k (1 + o(1)) \binom{n+2k-i}{i} 3^i W^2_{k-i} 
	\end{align*}

	% TODO: These computations only work for the diagonal case.
	% TODO: The lower bound is too weak for the straight case.
\end{proof}


==> notes/aztec_diamond_width.tex <==
%!TEX root = ../main.tex
\section{Aztec Diamond width Property}
We will prove that nearly antipodal points in the Aztec Diamond satisfy the hypothesis of \cref{t:long_cycle_bound_subgraph}.
To be precise, let $A_k$ denote the Aztec Diamond of size $k$, let $R,P$ be two points on the boundary of $A_k$. Let $Q$ be the antipodal point of $P$. Suppose that there is a partion with boundary size $6k + Ck^{(1-\epsilon)}$ whose endpoints are precisely $R,P$. We will assume without loss of generality that $P = (n_1, n_2) \ge (0,0)$. We first have the following lemma:

\begin{lemma}
	\label{l:aztec_partition_width}
	For the points $P,R$ described above, the Aztec Diamond $A_k$ is $(l, 16l + 4Ck^{(1-\epsilon)},0)$-wide.
\end{lemma}
\begin{proof}
	Note that all the points between $(-k,0)$ and $(0,-k)$ in $\partial A_k$ are at distance $k \pm 1$ from $P$. Thus, if $R$ is any point in the third quadrant, then $R$ and $Q$ can be at most $Ck^{1-\epsilon} + 1$ distance away, since otherwise for any partition, the boundary of one of the parts is larger than $4k + C^{1-\epsilon} + 1 + k - 1$, which is a contradiction.

	Let $R = (m_1,m_2) \le (0,0)$. Consider the lattice box $\Gamma = \mathcal{R}(R,P)$. The number of points on the boundary $\partial A_k$ that are in $\Gamma$ is at most $2 \abs{m_1-n_1} + 2 \abs{m_2 - n_2}$, which is $2 \dist(Q,R) \le Ck^{(1-\epsilon)}$. Further, any path of length $2l$ larger than the shortest path from $R$ to $P$ must be contained in a $\Gamma' = \mathcal{R}(R-(l,l), P+(l,l))$, which includes additional $16l$ boundary points of $A_k$ as compared to $\Gamma$. Any path contained in $\Gamma'$ hence can only intersect $\partial A_k$ in at most $16l + Ck^{(1-\epsilon)}$ points.

	If $R = (-m_1,m_2)$ is in the second quadrant, $m_1 + m_2 = k$, and the distane between $R$ and $P$ is 
	\[ m_1 + n_1 + \abs{n_2 - m_2} = m_1 + n_1 + \max(n_2,m_2) - \min(n_2,m_2) \ge 2k+1 - 2 \min(n_2,m_2) \]
	Further, length of the lower boundary of $A_k$ between $P$ and $R$ is $4k + n_2 + m_2$, and hence boundary of the lower partition is at least $6k + \abs{n_2 - m_2}$, which implies that
	\[ \abs{n_2 - m_2} \le  Ck^{(1-\epsilon)} \]
	The lattice box $\Gamma = \mathcal{R}(R,P)$ contains at most $2\abs{n_2 - m_2} + 4$ points on the boundary $\partial A_k$. By similar argument to above, we can conclude that any path of length $2l$ larger than the shortest path can intersect the boundary $\partial A_k$ in at most
	\[ 2\abs{n_2 - m_2} + 16l + 4 \le 16k + 4Ck^{(1-\epsilon)} \]
	points.

	The case when $R$ is in the fourth quadrant is handled similarly to the case when $R$ is in the second quadrant. This proves that in all cases, the Aztec Diamond is $(l, 16l + 4Ck^{(1-\epsilon)}, 0)$-wide. 
\end{proof}


==> notes/binomial_bounds.tex <==
For $-\frac{n}{2} \le x \le n$ and $k < \frac{n}{10}$, we have the upper bound
\begin{align*}
	\binom{n+x}{k}
	& \le \sqrt{\frac{n+x}{n+x-k}} \frac{1}{e^k k!} \brac{\frac{n+x}{n+x-k}}^{n+x-k} (n+x)^k \exp\brac{\frac{1}{12(n+x)} - \frac{1}{12(n+x-k) + 1}} \\
	& \le \frac{n^k}{e^k k!} \brac{1 + \frac{k}{{n+x-k}}}^{n+x-k + \frac{1}{2}} \brac{1 + \frac{x}{n}}^k \exp\brac{\frac{-k}{60 n^2}} \\
	& \le \frac{n^k}{k!} \exp\brac{-k + k + \frac{k}{2(n+x-k)} + \frac{kx}{n} - \frac{k}{60 n^2}} \\
	& \le \frac{n^k}{k!} \exp\brac{\frac{2k + kx}{n} - \frac{k}{60n^2}}
\end{align*}
On the other hand, we have the lower bound
\begin{align*}
	\binom{n+x}{k}
	& \ge \sqrt{\frac{n+x}{n+x-k}} \frac{1}{e^k k!} \brac{\frac{n+x}{n+x-k}}^{n+x-k} (n+x)^k \exp\brac{\frac{1}{12(n+x) + 1} - \frac{1}{12(n+x-k)}} \\
	& \ge \frac{n^k}{e^k k!} \brac{1 + \frac{k}{{n+x-k}}}^{n+x-k + \frac{1}{2}} \brac{1 + \frac{x}{n}}^k \exp\brac{\frac{-2 k}{n^2}} \\
	& \ge \frac{n^k}{k!} \exp\brac{-k + \brac{n+x-k + \frac{1}{2}} \cdot \brac{\frac{k}{n+x}} + k \cdot \frac{x}{n+x} - \frac{2 k}{n^2}} \\
	& \ge \frac{n^k}{k!} \exp\brac{\frac{-2k^2 + k + 2kx}{2(n+x)} - \frac{2 k}{n^2}}
\end{align*}
Combining the two, we get the bound
\begin{equation}
	\label{eq:binomial_bound_sterling}
	\frac{n^k}{k!} \exp\brac{\frac{-k^2}{n+x} + \frac{k + 2kx}{2(n+x)} - \frac{2k}{n^2}} \le \binom{n+x}{k} \le \frac{n^k}{k!} \exp\brac{\frac{k + 2kx}{2n} - \frac{k(x-k+1)}{n^2}}
\end{equation}


==> notes/paths_in_grid.tex <==
% !TEX_root = ../notes.tex
% Paths and Walks Notes

% Old second moment proofs without coupling
% Moved on:
% Last edited: 

\begin{lemma}
\label{l:k_cons_prob_old}
	Let $k, l \in \N$ and $1 \ge q > p > 0$, $1 \ge \epsilon > 0$ be reals. Let $a_1, \ldots, a_{l+k-1}$ be random variables such that
	\[ q > \pr{a_i = 1 \st a_{i-1}, \ldots, a_1} > p \qquad \forall i\]
	Then, given that
	\[ \frac{q}{p} \le 1 + \frac{\epsilon}{2k(2 + \epsilon)} \]
	\[ l \ge \frac{10k p^{-k}}{\epsilon} \]
	then $a_1, \ldots, a_{l+k-1}$ contains a continuous subsequence of $1$'s of length $k$ with probability $1 - \epsilon$.
\end{lemma}
\begin{proof}
	Let $X_i = 1$ if $a_j = 1$ for $i \le j < i + k$ and $0$ otherwise. We need to show that if given constraints are satisfied, then
	\[ \pr{\sum_{i=1}^{l} X_i = 0} < \epsilon \]
	First, observe that 
	\begin{align*}
		\pr{X_i} & = \pr{a_i = 1, \ldots a_{i+k-1} = 1}\\
						 & = \pr{a_{i+k-1} = 1 \st a_{i+k-2} \ldots a_i} \pr{a_i = 1, \ldots, a_{i+k-2} = 1}\\
						 & > p \pr{a_i = 1, \ldots a_{i+k-2} = 1}\\
						 & > p^k \tag*{by induction}
	\end{align*}
	Similarly, we have the upper bound $\pr{X_i} \le q^k$. Therefore, $lq^k > \ex{\sum_{i=1}^{l} X_i } > lp^k$. To get a bound on the required probability, we will use the chebyshev's inequality. First, we will bound the variance. Let $T_i = \set{i, i+1, \ldots, i+k-1}$. Notice that if $i \le j$ and $\abs{T_i \cap T_j} = t$, then the argument above shows that
	\[ \ex{X_iX_j} = \pr{X_i = 1, X_j = 1} \in \brac*{p^{2k - t}, q^{2k - t}} \]
	Let $X = \sum_{i=1}^l X_i$. Then
	\begin{align*}
		\ex{X^2} - \ex{X}^2
		& = \sum_{i,j} \ex{X_iX_j} - \ex{X_i}\ex{X_j} \\
		& = \sum_{t = 0}^k 2 \sum_{\substack{i \le j \\ \abs{T_i \cap T_j} = t}} \ex{X_i X_j} - \ex{X_i} \ex{X_j}\\
		& < \sum_{t = 1}^k 2l \brac{q^{2k-t} - p^{2k}} + l^2 \brac{q^{2k} - p^{2k}}\\
		& < 2lkq^k + l^2 q^{2k}
	\end{align*}
	Now, using chebyshev's bound, we get
	\begin{align*}
		\pr{X = 0} & \le \pr{\abs{X - \ex{X}} \ge \ex{X}} \\
							 & \le \frac{\ex{\brac{X - \ex{X}}^2}}{\ex{X}^2} \\
							 & = \frac{\ex{X^2} - \ex{X}^2}{\ex{X}^2} \\
							 & < \frac{2lkq^k + l^2 q^{2k}}{l^2 p^{2k}} \\
							 & = \frac{2kq^k}{lp^{2k}} + \frac{q^{2k} - p^{2k}}{p^{2k}}
	\end{align*}
	Let $\frac{q}{p} = 1 + \delta$. Then
	\[ \frac{q^{2k} - p^{2k}}{p^{2k}} = (1 + \delta)^{2k} - 1 \le \sum_{i=1}^{2k} \binom{2k}{i} \delta^{i} \]
	Assuming that $2k\delta \le t \le 1$, we have 
	\[ \binom{2k}{i+1} \delta^{i+1} = \binom{2k}{i} \frac{2k - i}{i+1} \delta^{i+1} \le \binom{2k}{i} \delta^i (2k\delta) \le t \binom{2k}{i} \delta^i \]
	Therefore, by induction, it follows that
	\[ \sum_{i=1}^{2k} \binom{2k}{i} \delta^i \le 2k \delta (1 + t + \ldots + t^{2k-1}) \le \frac{2k \delta}{1 - t} \]
	If $\delta \le \frac{\epsilon}{2k(2+\epsilon)}$, then for $t = \frac{\epsilon}{2 + \epsilon}$, we have $2k \delta \le t$ and $\frac{2k\delta}{1 - t} \le \frac{t}{1-t} = \frac{\epsilon}{2}$. This implies that $\frac{q^{2k} - p^{2k}}{p^{2k}} < \frac{\epsilon}{2}$.
	On the other hand, 
	\[ \frac{2kq^{2k}}{lp^{2k}} = \frac{2k (1+\delta)^k}{lp^k} \le \frac{2k e^{\delta k}}{lp^k} \le \frac{5k}{lp^k} \le \frac{\epsilon}{2} \]
	where the last two inequalities follows using $2k\delta < \epsilon \le 1$ and $l > \frac{10kp^{-k}}{\epsilon}$. Putting the two results together, we get that
	\[ \pr{X = 0} < \epsilon \]
	as required.
\end{proof}

\begin{lemma}
\label{l:stright_segments_bound}
	Let $k \in \N$ and $\epsilon > 0$ be given. Then for any point $P = (n_1,n_2)$ with $n_1 + n_2 = n$, a shortest path from $O = (0,0)$ to $P$ drawn uniformly at random has $c_{k,\epsilon} n$ many straight segments of length at least $k$ as $n \to \infty$.
\end{lemma}
\begin{proof}
	Any shortest path from $O$ to $P$ can be denoted as a sequence of exactly $n_1$ right moves and exactly $n_1$ up moves. Let $a_1 \ldots a_n$ denote the path written as a sequence of these moves. If $a_1 \ldots a_i$ has exactly $\lambda_1$ right moves and $\lambda_2$ up moves, then the probability that $a_{i+1}$ is a right move is $\frac{n_1 - \lambda_1}{n - \lambda_1 - \lambda_2}$, and the probability that $a_{i+1}$ is an up move is $\frac{n_2 - \lambda_2}{n - \lambda_1 - \lambda_2}$.

	Let $l \in \N$ and $1 > \alpha,\beta, \gamma > 0$ be reals. Let $S_i = \set{(i-1)l + 1, \ldots, il}$. Given the values of $a_1, \ldots, a_{(i-1)l}$, we can find a preffered direction, either up or right, for which $\pr{a_{(i-1)l+1} \st a_1, \ldots, a_{(i-1)l}} > \frac{1}{2}$. Now, we generate a new sequence $b_1, \ldots, b_l$ of length $l$ such that $b_j$ is $1$ if $a_{(i-1)l + j}$ is the preffered direction, and $b_j = 0$ otherwise. Then, we have that 
	\[ p + \frac{l}{\beta n} > \pr{b_j = 1 \st b_{j-1}, \ldots, b_1} > p - \frac{l}{\beta n} \]
	for some value of $p \ge 0.5$. Let $Y_i$ be the event that there is a straight segment of length $k$ in the set $\set{a_j \st j \in S_i}$. This implies that there are $k$ consecutive ones in the sequence $b_j$. Suppose that $l$ satisfies
	\[ l > 10 k 4^k \frac{1}{\epsilon_1} \]
	and $n$ is large enough so that
	\[ \epsilon_1 \ge \frac{40kl}{\beta n} \]
	conditions for \cref{l:k_cons_prob_old} are satisfied. Therefore, $\pr{Y_i \st a_1, \ldots, a_{(i-1)l}} > 1 - \epsilon_1$. The condition on $n$ is required to ensure that 
	\[ \frac{p + \frac{l}{\beta n}}{p - \frac{l}{\beta n}} = 1 + \frac{\frac{2l}{\beta n}}{p - \frac{l}{\beta n}} = 1 + \frac{8l}{\beta n} \le 1 + \frac{\epsilon_1}{2k (2 + \epsilon_1)} \]
	which satisfies the condition on $\delta$ in \cref{l:k_cons_prob_old}. Therefore, we have a bound: 
	\[ 1 \ge \pr{Y_i} \ge 1 - \epsilon_1 \]
	Let $t = \frac{(1 - \beta) n}{l}$, and let $Y = \sum_{i=1}^{(1 - \beta)n/l} Y_i$. Then using chebyshev's inequality, we get the bound
	\begin{align*}
	  \pr{\abs{Y - \ex{Y}} > \alpha t}
		& \le \frac{\sum_{1 \le i,j \le t}\ex{Y_iY_j} - \ex{Y_i}\ex{Y_j}}{\alpha^2 t^2} \\
		& \le \frac{t^2(1 - (1 - \epsilon_1)^2)}{\alpha^2 t^2} \\
		& \le \frac{2 \epsilon_1}{\alpha^2} 
	\end{align*}
	since $\ex{Y} \ge (1 - \epsilon_1)t$, we get that
	\[ \pr{Y < \frac{(1 - \epsilon_1 - \alpha)(1-\beta)n}{l}} \le \frac{2 \epsilon_1}{\alpha^2} \]
	ensuring that $\epsilon > \frac{2\epsilon_1}{\alpha^2}$ gives us the result.

	We can pick $\alpha$ and $\beta$ to be any constnats, for example, $\alpha = \beta = 1/2$ will give us
	\[ c_{k,\epsilon} = \frac{\epsilon}{300k4^k} \]
\end{proof}

% k-length segments coupling proofs
% Moved on: 12:51 Friday 12th Nov
% Last modified 12:51 Friday 12th Nov

\begin{lemma}
\label{l:k_cons_prob}
	Let $k,l \in \N$ and $1 \ge p > 0, 1 \ge \epsilon > 0$ be reals. Let $a_1, \ldots, a_{l+k-1}$ be random variables such that
	\[ \pr{a_i = 1 \st a_{i-1}, \ldots, a_1} > p \qquad \forall i \]
	Then, given that
	\[ l \ge \frac{2kp^{-k}}{\epsilon} \]
	then $a_1, \ldots, a_{l+k-1}$ contains a continuous subsequence of $1$'s of length $k$ with probability $1-\epsilon$.
\end{lemma}
\begin{proof}
	We will prove this by a coupling argument. Consider a sequence $b_1, \ldots, b_{l+k-1}$ such that $b_i = 1$ with probability $1$. We couple this with $a_i$ using following process: given $a_1, \ldots, a_{i-1}$, we draw a number $x$ uniformly at random from $[0,1]$. If $x \le p$, we set $b_i = 1$ and if $x \le p_i$, we set $a_i = 1$. This coupling ensures that if $b_i = 1$, then $a_i = 1$ since $\pr{a_i = 1 \set a_{i-1}, \ldots, a_1} = p_i > p$. Therefore, probability that $b_i$ contains a consecutive subsequence of $k$ ones is a lower bound for the probably that $a_i$ contains a consecutive subsequence of $k$ ones.

	Now, we bound the probability that $b_i$ contains a consecutive subsequence of $k$ ones. Let $X_i = 1$ if $b_j = 1$ for $i \le j < i + k$ and $X_i = 0$ otherwise. We need to show that if given constraints are satisfied, then
	\[ X = \pr{\sum_{i=1}^{l} X_i = 0} < \epsilon \]
	Since $b_i$ are independent, $\pr{X_i = 1} = p^k$. Let $T_i = \set{i, i+1, \ldots, i+k-1}$. If $i \le j$ and $\abs{T_i \cap T_i} = t$, then
	\[ \ex{X_i X_j} = \pr{X_i = 1, X_j = 1} = p^{2k - t} \]
	We will now use chebyshev's inequality to show concentration of $X_i$. $\ex{X} = lp^k$. First, we compute the variance.
	\begin{align*}
		\ex{X^2} - \ex{X}^2
		& = \sum_{i,j} \ex{X_iX_j} - \ex{X_i}\ex{X_j} \\
		& = \sum_{t = 0}^k 2 \sum_{\substack{i \le j \\ \abs{T_i \cap T_j} = t}} \ex{X_i X_j} - \ex{X_i} \ex{X_j}\\
		& < \sum_{t = 1}^k 2l \brac{p^{2k-t} - p^{2k}}\\
		& < 2lkp^k
	\end{align*}
	Now, using chebyshev's bound, we get
	\begin{align*}
		\pr{X = 0} & \le \pr{\abs{X - \ex{X}} \ge \ex{X}} \\
							 & \le \frac{\ex{\brac{X - \ex{X}}^2}}{\ex{X}^2} \\
							 & = \frac{\ex{X^2} - \ex{X}^2}{\ex{X}^2} \\
							 & < \frac{2lkp^k}{l^2 p^{2k}} \\
							 & = \frac{2k}{lp^{k}}
	\end{align*}
	This gives us the result provided that $l \ge \frac{2kp^{-k}}{\epsilon}$.
\end{proof}

\begin{lemma}
\label{l:stright_segments_bound}
	Let $k \in \N$ and $\epsilon > 0$ be given. Then for any point $P = (n_1,n_2)$ with $n_1 + n_2 = n$, a shortest path from $O = (0,0)$ to $P$ drawn uniformly at random has $c_k n$ many straight segments of length at least $k$ as $n \to \infty$.
\end{lemma}
\begin{proof}
	Any shortest path from $O$ to $P$ can be denoted as a sequence of exactly $n_1$ right moves and exactly $n_2$ up moves. Let $a_1 \ldots a_n$ denote the path written as a sequence of these moves. If $a_1 \ldots a_i$ has exactly $\lambda_1$ right moves and $\lambda_2$ up moves, then the probability that $a_{i+1}$ is a right move is $\frac{n_1 - \lambda_1}{n - \lambda_1 - \lambda_2}$, and the probability that $a_{i+1}$ is an up move is $\frac{n_2 - \lambda_2}{n - \lambda_1 - \lambda_2}$.

	Let $l \in \N$ and $1 > \alpha,\beta, \gamma > 0$ be reals. Let $S_i = \set{(i-1)l + 1, \ldots, il}$. Given the values of $a_1, \ldots, a_{(i-1)l}$, we can find a preffered direction, either up or right, for which $\pr{a_{(i-1)l+1} \st a_1, \ldots, a_{(i-1)l}} > \frac{1}{2}$. Now, we generate a new sequence $b_1, \ldots, b_l$ of length $l$ such that $b_j$ is $1$ if $a_{(i-1)l + j}$ is the preffered direction, and $b_j = 0$ otherwise. Then, we have that 
	\[ p + \frac{l}{\beta n} > \pr{b_j = 1 \st b_{j-1}, \ldots, b_1} > p - \frac{l}{\beta n} \]
	for some value of $p \ge 0.5$. Let $Y_i$ be the event that there is a straight segment of length $k$ in the set $\set{a_j \st j \in S_i}$. This implies that there are $k$ consecutive ones in the sequence $b_j$. Suppose that $l$ satisfies
	\[ l = 2 k (2 + \alpha)^k \frac{1}{\epsilon_1} \]
	and $n$ is large enough so that
	\[ \frac{1}{2 + \alpha} \ge \frac{1}{2} - \frac{1}{\beta n} \]
	conditions for \cref{l:k_cons_prob} are satisfied. Therefore, $\pr{Y_i \st a_1, \ldots, a_{(i-1)l}} > 1 - \epsilon_1$.
	Note that the condition above is satisfied if $\alpha \beta n \ge 5$. 

	Now, we do same coupling arguement in the proof above, and couple $Y_i$ with $Z_i$ which are drawn independently such that $\pr{Z_i = 1} = 1 - \epsilon_1$. Using the exact same coupling as in \cref{l:k_cons_prob} and chernoff's inequality, we get:
	\begin{align*}
		\pr{Y \le (1 - \delta) \ex{Z}}
		& \le \pr{Z \le (1 - \delta) \ex{Z}} \\
		& \le \exp\brac{- \frac{\delta^2\ex{Z}}{2}} \\
		& \le \exp\brac{- \frac{\delta^2(1 - \epsilon_1) t}{2}}
	\end{align*}
	since $\ex{Z} = (1 - \epsilon_1)t$, we get that
	\[ \pr{Y < \frac{(1 - \delta)(1 - \epsilon_1)(1-\beta)n}{l}} \le \exp\brac{-\frac{\delta^2(1-\epsilon_1)(1-\beta)n}{2l}} = \exp\brac{-\frac{\delta^2 \epsilon_1 (1 - \epsilon_1)(1 - \beta)n}{4k(2 + \alpha)^k}} \]

	We now set $\epsilon_1 = 0.5$ and choose $\delta = \alpha = \beta = \frac{1}{\log n}$ to get that 
	\[ \pr{Y < (1 - o(1)) \frac{n}{4k2^k}} \le \epsilon \]
	for $n$ such that
	\[ \frac{n}{4k4^k\log^2 n} > - \log \epsilon \]
	% TODO: We can potentially tweak the constants here to get a result for bigger ranges of $n$.
\end{proof}

% Proof of the advanced extension lemma:
% This gives a better bound than the basic version, but basic version suffices for the paper.
% Moved on: 
% Last modified: 

% TODO: write this proof using algorithmic section
\begin{lemma}
	\label{l:path_extension_advanced}
	For any $k$ and $1 > \epsilon \ge 0$,
	\[ P_k \ge (1 -	\epsilon) P_0 \frac{n^k 2^{-k}}{k!} \exp\brac{\frac{- 4 k \log n - k \sqrt{-n \log \epsilon} + k^2}{n}} \]
\end{lemma}
\begin{proof}
	We do this by constructing a family of these paths. Consider a shortest path $S$ from $O$ to $P$. This path can be represented by a sequence $a_1, \ldots, a_n$ of $U$ and $R$ symbols of length $n$. From this path of length $n$, we can construct a path of length $n + 2k$ as follows:
	\begin{enumerate}[nosep]
		\item For each $i$ such that $a_i = a_{i+1}$, we fix a number $u_i \in \Z_{\ge 0}$ such that $\sum u_i = k$. We let $u_i = 0$ if $a_i \neq a_{i+1}$.
		\item For each $i$, we add $u_i$ moves in the \emph{wrong} perpendicular direction. For example, if $a_i = a_{i+1} = U$, then we add $u_i$ $L$ symbols in between $a_i$ and $a_{i+1}$.
		\item For every $i$ such that $a_i \neq a_{i+1}$, we reset the path by adding appropriate moves in the \emph{correct} direction, so that we go through the same point again.
	\end{enumerate}
	Here, $U,R$ are the \emph{correct} directions and $D, L$ are the \emph{wrong} directions. For example, a straight line path from $(0,0)$ to $(5,0)$ with $u_1 = 1$, $u_2 = 0$, $u_3 = 2$, $u_4 = 1$ becomes the path 
	\[ (0,0) \to (1,0) \to (1,-1) \to (2,-1) \to (2, -3) \to (3,-3) \to (3,-4) \to (4,-4) \to (5,-4) \to (5,0) \]
	\begin{figure}
		\centering
		\includesvg[width=0.2\textwidth]{extension_1/small_base.svg}
		\hspace{3cm}
		\includesvg[width=0.2\textwidth]{extension_1/small_ext.svg}
		\caption{Modifying the path with $u = (1,0,2,1)$}
		\label{f:extension_1_small}
	\end{figure}
	\begin{figure}
		\centering
		\includesvg[width=0.2\textwidth]{extension_1/large_base.svg}
		\hspace{3cm}
		\includesvg[width=0.2\textwidth]{extension_1/large_ext.svg}
		\caption{Modifying the path with $u = (1,0,2,0,1,0,1)$}
		\label{f:extension_1_large}
	\end{figure}
	This extension corresponds to $k = 4$, and length of extended path is $13$. This is illustrated on a straight line path in \cref{f:extension_1_small}, and in a slightly more general setting in \cref{f:extension_1_large}.
	It is clear that this construction creates a walk of length $n + 2k$ without backtracking. We claim that it is in fact a path.

	% TODO: write a partitioning argument to complete the proof
	% TODO: add figures to show an example.
	\asnote{Need to finish a boxing argument to prove that these are all paths}

	Therefore, every path with $l$ straight points (where $a_i = a_{i+1}$) can be extended to a path of length $k$ in at least $\binom{l+k}{k}$ many ways. 
	Using \cref{l:straight_path}, for $(1-\epsilon)$ fraction of paths, there are $\frac{n}{2} - 2\log n - \sqrt{-n \log \epsilon}$ places where $u_i$ can be non-zero! Therefore, we get a lower bound
	\[ P_k \ge (1 - \epsilon) P_0 \binom{\frac{n}{2} - 2 \log n - \sqrt{-n \log \epsilon} + k}{k} \]
	We can simplify the expression above. For $a,b = o(n)$, we have 
	When $k = o(n)$, we can further lower bound this by
	\[ P_k \ge (1 -	\epsilon) P_0 \frac{n^k 2^{-k}}{k!} \exp\brac{\frac{- 4 k \log n - k \sqrt{-n \log \epsilon} + k^2}{n}} \]
	Which proves the required claim. Further, for $k = o(\sqrt{n/f(n)})$, we can set $\epsilon = \frac{1}{f(n)}$, to get that $P_k \ge (1 - o(1)) P_0 \frac{n^k2^{-k}}{k!}$ for an function $f$ such that $\lim_{n \to \infty} f(n) = \infty$.
\end{proof}



==> sections/grid_spanning_tree.tex <==
% !TEX root = ../main.tex
\section{Number of Spanning Trees in a Rectangular Grid}
\label{s:grid_spanning_tree}
Consider a $\sqrt{p} \times \sqrt{q}$ grid graph. Let $\tau(p,q)$ denote the number of spanning trees in the $p \times q$ grid. From \cite{rote2005spanning}, we know that $\tau(p,q) \le 3.53^{pq}$. Define 
\begin{equation}
	\label{e:def_alpha}
	\alpha(p,q) = \frac{1}{pq} \log \tau(p,q)
\end{equation}
For any $p,q$ note that $0 \le \alpha \le 3.53$. 

\begin{lemma}
	\label{l:alpha_lim}
	$\lim_{p,q \to \infty} \alpha(p,q)$ exists.
\end{lemma}
\begin{proof}
	First, we will show this convergence for square grids. Since value of $\alpha(n,n)$ is bounded, the set $\set*{\alpha(n,n) \st n \in \N}$ has a limit point. To show convergence, we need to show that there is a unique limit point. Suppose not. Then there are at least two limit points $A,B$ with subsequences $n_1, n_2, \ldots$ and $m_1, m_2, \ldots$ such that $\lim_{i \to \infty} \alpha(n_i,n_i) = A$ and $\lim_{j \to \infty} \alpha(m_j,m_j) = B$.

	Now, for any $p,q > n$, we can divide the rectangle of size $p \times q$ into squares of size $n$. Since we can merge spanning trees in each of the $n \times n$ squares into a spanning tree on the $p \times q$ rectangle, this gives us a lower bound:
	\begin{align*}
		pq \, \alpha(p,q) & \ge \floor{\frac{p}{n}} \floor{\frac{q}{n}} n^2 \, \alpha(n,n) \\
											& \ge pq \brac{1 - \frac{n}{p}} \brac{1 - \frac{n}{q}} \alpha(n,n) \\
		\Rightarrow \alpha(p,q) &\ge \brac{1 - \frac{n}{p}} \brac{1 - \frac{n}{q}} \alpha(n,n) \labeleqn{e:rectangle_lb}
	\end{align*}

	Choosing $p = q = m_j \gg n_i$, we get that $B \ge A$, and choosing $p = q = n_i \gg m_j$ gives us that $A \ge B$, and therefore $A = B$. Hence, $\lim_{n \to \infty} \alpha(n,n)$ exists.

	To get an upper bound, consider a spanning tree on the whole rectangle of size $p \times q$. For a fixed square of size $n \times n$ in this rectangle, this tree gives rise to a forest. Note that it might have more than one connected component. But, we can convert each forest into a tree by adding edges on the boundary in the following manner: we start at the left top vertex, go clockwise, and add any edge whose endpoints are in different connected components until the forest is connected.

	Further, given a tree on the $n \times n$ grid with $m$ edges on the boundary, it could have originated from at most $2^m$ different forests. Therefore, we can bound number of these forests as $2^n \tau(n,n)$. Given a rectangle of size $p \times q$, it can be covered using $\ceil*{\frac{p}{n}} \ceil*{\frac{q}{n}}$ squares of size $n \times n$, and then the above argument gives us an upper bound:
	\begin{align*}
		\tau(p,q) & \le \brac{2^{4n} \tau(n,n)}^{\ceil*{\frac{p}{n}} \ceil*{\frac{q}{n}}} \\
		\Rightarrow pq \, \alpha(p,q) & \le \ceil{\frac{p}{n}} \ceil{\frac{q}{n}} \brac{4n \log 2 + n^2 \, \alpha(n,n)} \\
		\Rightarrow \alpha(p,q) & \le \brac{1 + \frac{n}{p}} \brac{1 + \frac{n}{q}} \brac{\frac{4 \log 2}{n} + \alpha(n,n)} \labeleqn{e:rectangle_ub}
	\end{align*}

	Choosing $n \ll p,q$ such that $n \to \infty$ as $p,q \to \infty$ (for example $n^2 = \min(p,q)$), we get that 
	\[ (1 - o(1)) \alpha(n,n) \le \alpha(p,q) \le (1 + o(1)) \alpha(n,n) \]
	using \Cref{e:rectangle_lb,e:rectangle_ub}. This proves the lemma.
\end{proof}


\begin{lemma}
	\label{l:convergence_rate}
	Suppose 
	\[ \lim_{n \to \infty} \alpha(n,n) = \alpha \] 
	which exists because of \Cref{l:alpha_lim}. Then $\alpha(n,n)$ converges with rate $1/n$, that is
	\[ A \ge \alpha(n,n) \ge \alpha - O(1/n) \]
\end{lemma}
\begin{proof}
	Using \Cref{e:rectangle_lb,e:rectangle_ub}, we get
	\[ \brac{1 - \frac{n}{p}} \brac{1 - \frac{n}{q}} \alpha(n,n) \le \alpha(p,q) \le \brac{1 + \frac{n}{p}} \brac{1 + \frac{n}{q}} \brac{\alpha(n,n) + \frac{4 \log 2}{n}} \]
	taking limit as $p,q \to \infty$, we get
	\[ \alpha(n,n) \le \alpha \le \alpha(n,n) + \frac{4 \log 2}{n} \]
	this gives us the result

	\begin{equation}
		\label{e:convergence_rate}
		\alpha - \frac{4 \log 2}{n} \le \alpha(n,n) \le \alpha
	\end{equation}
\end{proof}

\begin{lemma}
	\label{l:alpha_max}
	For a fixed $n$ and any $p,q$ such that $pq = n$,
	\[ \alpha(\sqrt{n},\sqrt{n}) \ge \alpha(p,q) \]
\end{lemma}


==> sections/shrinking_lattice_spaning_trees.tex <==
% !TEX root = ../main.tex
\section{Number of Spanning Trees in Subsets of the Grid}
\label{s:shrinking_lattice}
In this section, we look at a slightly different setting where we fixed a closed curve containing origin, and look at the grid of squares $\frac{1}{n} \times \frac{1}{n}$. For a closed curve $\Gamma$, we define $\tau_\Gamma(n)$ to be the number of spanning trees in the grid graph in the interior of $\Gamma$. Define $\beta_\Gamma(n) = \frac{1}{n^2} \log \tau_\Gamma(n)$. Further, we define $P(\Gamma)$ to be the length (perimeter) of $\Gamma$ and $A(\Gamma)$ to be the area in  the interior of $\Gamma$. Whenever it is clear what $\Gamma$ is, we will drop $\Gamma$ from the notation.

\begin{lemma}
	For any closed curve $\Gamma$ such that $P(\Gamma)$ and $A(\Gamma)$ are finite, then $\lim_{n \to \infty} \beta_\Gamma(n)$ exists and further
	\begin{equation}
		\lim_{n \to \infty} \beta_\Gamma(n) = \beta_\Gamma = A(\Gamma) \alpha
	\end{equation}
\end{lemma}
\begin{proof}
	Since we are fixing $\Gamma$, we will drop $\Gamma$ from the notation for this proof. Consider the grid of size $\frac{1}{n}$. Any squares in this grid that touches interior of $\Gamma$ is completely contained in a strip of width $\frac{2}{n}$ around $\Gamma$ on both sides. Note that the total area of the strip is $\frac{4P}{n}$. Therefore there are at most $4Pn$ of these squares which covers the entire perimeter. Similarly, any squares that intersect with the interior of $\Gamma$ contained inside $\Gamma$ and this strip of size $\frac{2}{n}$ around it. The total area is at most $A + \frac{2P}{n}$, which implies that there are at most $An^2 + 2Pn$ squares which can intersect the interior of $\Gamma$. All these squares completely cover the area of $\Gamma$ and hence there are at least $An^2$ such squares. Among these $An^2$ squares, there can be at most $4Pn$ squares which touch the curve $\Gamma$. This implies that we can pack at least $An^2 - 4Pn$ squares of size $\frac{1}{n} \times \frac{1}{n}$ which are completely inside $\Gamma$, and cover it using at most $An^2 + 2Pn$ squares of the same size.

	Now consider the grid of size $\frac{1}{m}$. Each of the squares above of size $\frac{1}{n}$ which align with the grid of size $\frac{1}{n}$ contains $\floor{\frac{m}{n}}^2$ squares in the smaller grid. This gives us a lower bound:
	\begin{align*}
		\tau_\Gamma(m) & \ge \tau\brac{\floor{\frac{m}{n}},\floor{\frac{m}{n}}}^{\brac{An^2 - 4Pn}} \\
		\Rightarrow \beta_\Gamma(m) & \ge \frac{1}{m^2} \brac{An^2- 4Pn} \log \tau\brac{\floor{\frac{m}{n}},\floor{\frac{m}{n}}} \\
																& \ge \frac{1}{m^2} \floor{\frac{m}{n}}^2 \brac{An^2- 4Pn} \alpha\brac{\floor{\frac{m}{n}},\floor{\frac{m}{n}}}\\
																& \ge \brac{1 - \frac{n}{m}}^2 \brac{A- \frac{4P}{n}} \alpha\brac{\floor{\frac{m}{n}},\floor{\frac{m}{n}}} \labeleqn{e:curve_lb}
	\end{align*}

	Each square of $\frac{1}{n} \times \frac{1}{n}$ is contained in a grid of size $\ceil{\frac{m}{n}} \times \ceil{\frac{m}{n}}$ using squares of size $\frac{1}{m} \times \frac{1}{m}$. Using the forest argument that leads to \Cref{e:rectangle_ub}, we get an upper bound as well:
	\begin{align*}
		\tau_\Gamma(m) & \le \brac{2^{4 \ceil{\frac{m}{n}}} \tau\brac{\ceil{\frac{m}{n}},\ceil{\frac{m}{n}}}}^{\brac{An^2 + 2Pn}} \\
		\Rightarrow \beta_\Gamma(m) & \le \frac{1}{m^2} \brac{An^2 + 2Pn} \brac{\log \tau\brac{\ceil{\frac{m}{n}},\ceil{\frac{m}{n}}} + 4 \ceil{\frac{m}{n}} \log 2} \\
																& \le \brac{1 + \frac{n}{m}}^2 \brac{A + \frac{2P}{n}} \brac{\alpha\brac{\ceil{\frac{m}{n}},\ceil{\frac{m}{n}}} + \frac{4n\log 2}{m}}
																\labeleqn{e:curve_ub}
	\end{align*}

	Choosing $m \gg n \to \infty$, we get that $\lim_{n \to \infty} \beta_\Gamma(n)$ exists. Let this limit be $\beta_\Gamma$. Then taking the limit as $m \to \infty$ in \Cref{e:curve_lb,e:curve_ub}
	\[ \brac{A - \frac{4P}{n}} \alpha \le \beta_\Gamma \le \brac{A + \frac{2P}{n}}\alpha \]
	Since this holds for all $n$, $\beta_\Gamma = A \alpha$ which completes the proof.
\end{proof}

Note that the result above works only when the the area in the closed curve and its perimeter is finite. Now, we look at a more general setting where we look at a bounded set $S \subseteq \R^2$. We define $G_S(n)$ to be the subset of $\frac{1}{n} \times \frac{1}{n}$ lattice that is defined by the corners of all the squares in the lattice that intersect $S$. To be precise, the square is any set of the form $[\frac{a}{n}, \frac{a+1}{n}] \times [\frac{b}{n}, \frac{b+1}{n}]$ for some integers $a,b$. We define $\tau_S(n)$ to be number of spanning trees on $G_s(n)$.


==> sections/walks_in_grid.tex <==
% !TEX root = ../main.tex
\section{Number of Walks}
\label{s:number_of_walks}
We now get some exact expressions for number of walks on the grid in terms of binomial coefficients. We also provide some approximations for these values which are more useful in computations.
\begin{lemma}
	\label{l:number_of_walks}
	For any point $P = (n_1, n_2)$ such that $n_1 + n_2 = n$, the number of walks from $O = (0,0)$ to $P$ of length $n + 2t$ is given by
	\[ \binom{n + 2t}{t} \binom{n+2t}{n_1 + t} \]
\end{lemma}
\begin{proof}
	Let $W_t$ denote number of such walks. Note that any such path can be denoted as a sequence of symbols $U,D,L,R$ which denote moves in the corresponding directions. For a direction $Z \in \set{U,D,L,R}$, let $n_Z$ denote number of symbols signifying the direction that appear in the walk; then the walks from $O$ to $P$ are in bijection with the sequences over $\{U,D,L,R\}$ of length $n+2t$ for which $n_U - n_D = n_1$ and $n_R - n_L = n_2$.  Note then that $n_L+n_D=t$, $n_U+n_L=n_1+t$, and $n_R+n_D=n_2+t$.  There is a bijection from the set of these sequences $s$ to pairs of subsets $(X_s,Y_s)\subseteq [n+2t]$ where $|X_s|=t$ and $|Y_s|=n_1+t$ as follows.  Given such a sequence $s$, we can let $X_s$ be the set of indices with symbols $L$ or $D$, while $Y_s$ is the set of indices with symbols $U$ or $L$.  The sequence $s$ is recovered from the sets $X_s$ and $Y_s$ by assigning the symbol $U$ to indices in $X_s\setminus Y_s$, the symbol $L$ to indices in $X_s\cap Y_s$, the symbol $D$ to those in $Y_s\setminus X_s$, and the symbol $R$ to indices in neither $X_s$ nor $Y_s$.
	%where $\#S$ denotes number of occurrences of symbol $S$.
	%Fix $i,j$ such that $i + j = t$. Then number of walks such that $n_U = n_1 + i$, $n_D = i$, $n_R = n_2 + j$, $n_L = j$ is given by
	%\[ \frac{(n+2t)!}{(n_1+i)!i!(n_2+j)!j!} \]
	%summing up over $i,j$, we get the total number of walks to be
	%\begin{align*}
%		W_t = & \sum_{i+j=t} \frac{(n+2t)!}{(n_1+i)!i!(n_2+j)!j!} \\
%		= & \frac{(n+2t)!}{t!(n+t)!} \sum_{i+j=t} \frac{t!}{i!j!} \frac{(n+t)!}{(n_1+i)!(n_2+j)!} \\
%		= & \binom{n+2t}{t} \sum_{i+j=t} \binom{t}{i} \binom{n+t}{n_2+j} \\
%		= & \binom{n+2t}{t} \binom{n+2t}{n_2 + t} \tag*{Vandermonde's indentity} 
%	\end{align*}
%	This completes the proof.
\end{proof}
\begin{corollary}
	\label{l:number_of_cycles}
	Number of closed walks of length $2k$ on the grid is 
	\[ C_k = \binom{2k}{k}^2 \]
\end{corollary}
\begin{proof}
	We set $P = (0,0)$ in \Cref{l:number_of_walks} to get this result.
\end{proof}

The rate of growth of $W_t$ depends heavily on $n_1,n_2$. This is to compensate for the fact that $W_0$ itself is large when say $n_1 = n_2 = \frac{n}{2}$ and on the other hand, its very small when $n_1 = 0$ and $n_2 = n$, but the values get closer and closer as $t \to \infty$. We now get bounds on the rate of growth of $W_t$.
Since $W_0 = \binom{n}{n_1}$,
\[ W_t = W_0 \binom{n+2t}{t} \frac{(n+1) \cdots (n+2t)}{(n_1 + 1) \cdots (n_1 + t) (n_2 + 1) \cdots (n_2 + t)} \]
\asnote{can get weaker bounds when $t \neq o(n)$}
Assuming $t = o(n)$, \asnote{add binomial bounds here} gives us the upper bound
\[
	\brac{\frac{n^2}{n_1 n_2}}^t \exp{\brac{\frac{2t^2}{n}}}
	\ge \frac{(n+1) \cdots (n+2t)}{(n_1 + 1) \cdots (n_1 + t) (n_2 + 1) \cdots (n_2 + t)}
\] 
and the lower boundc
\[
	\frac{(n+1) \cdots (n+2t)}{(n_1 + 1) \cdots (n_1 + t) (n_2 + 1) \cdots (n_2 + t)}
	\ge (1 - o(1)) \brac{\frac{n^2}{n_1 n_2}}^t \exp{\brac{\frac{t^2}{n} - \frac{2t^2}{n_1} - \frac{2t^2}{n_2}}} 
\]
which holds since $(n_1 + 1) \cdots (n_1 + t) \le n_1^t \exp{\brac{\frac{1}{n_1} + \cdots + \frac{t}{n_1}}} \le n_1^t \exp{\brac{\frac{t^2}{2n_1}}}$.
Further, we have the following bounds on the binomial from \asnote{insert binomial bound here}
\[ \frac{n^t}{t!} \exp{\brac{\frac{4t^2 - t(t-1)}{4n}}} \le \binom{n + 2t}{t} \le \frac{n^k}{k!} \exp{\brac{\frac{-k(k-1)}{2n}}} \]
Putting all the three bounds together, we get
\begin{equation}
	\label{eq:walks_bounds}
	(1 - o(1)) \frac{n^t}{t!} \brac{\frac{n^2}{n_1n_2}}^t \exp{\brac{\frac{7t^2}{2n} - \frac{t^2}{2n_1} - \frac{t^2}{2n_2}}} W_0 \le W_t \le (1 + o(1)) \frac{n^t}{t!} \brac{\frac{n^2}{n_1 n_2}}^t \exp{\brac{\frac{7t^2}{n}}} W_0
\end{equation}

Note that the upper and lower bounds differ by $\exp(-t^2)$ in the worse case where $n_1 = 1$ and $n_2 = n-1$. In general, it feels like analysis of this case is easier, there is exactly one shortest path.


